Augmented Lagrangian methods for fully convex composite optimization

This paper is concerned with augmented Lagrangian methods for the treatment of fully convex composite optimization problems. We extend the classical relationship between augmented Lagrangian methods and the proximal point algorithm to the inexact and safeguarded scheme in order to state global primal-dual convergence results. Our analysis distinguishes the regular case, where a stationary minimizer exists, and the irregular case, where all minimizers are nonstationary. Furthermore, we suggest an elastic modification of the standard safeguarding scheme which preserves primal convergence properties while guaranteeing convergence of the dual sequence to a multiplier in the regular situation. Although important for nonconvex problems, the standard safeguarding mechanism leads to weaker convergence guarantees for convex problems than the classical augmented Lagrangian method. Our elastic safeguarding scheme combines the advantages of both while avoiding their shortcomings.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{amsfonts,amssymb}
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage{nicefrac}
\usepackage{graphicx}
\usepackage{xcolor}

% https://www.math.cmu.edu/~gautam/sj/blog/20171114-bibtex-doi.html
% since some DOIs might contain evil special characters
\RequirePackage{doi}

\definecolor{darkblue}{RGB}{0,102,153}

\usepackage{cite}

\usepackage{hyperref}
\hypersetup{colorlinks,
	citecolor=darkblue,
	linkcolor=darkblue,
	urlcolor=darkblue}

\usepackage[ruled,vlined,linesnumbered,algosection,algo2e]{algorithm2e} % Before cleveref

\usepackage[capitalize,noabbrev,nameinlink]{cleveref} % After hyperref

\usepackage{multirow}

\hyphenation{pro-xi-mal Lip-schitz boun-ded-ness}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{assum}[theorem]{Assumption}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{setting}{Setting}

% patch from https://tex.stackexchange.com/a/730164
\AddToHook{env/corollary/begin}{\crefalias{theorem}{corollary}}
\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}
\AddToHook{env/assum/begin}{\crefalias{theorem}{assum}}
\AddToHook{env/definition/begin}{\crefalias{theorem}{definition}}
\AddToHook{env/example/begin}{\crefalias{theorem}{example}}
\AddToHook{env/remark/begin}{\crefalias{theorem}{remark}}
\AddToHook{env/setting/begin}{\crefalias{theorem}{setting}}

% cref names
\crefname{assum}{Assumption}{Assumptions}
\crefname{setting}{Setting}{Settings}

% keyworkds and subclass
\newcommand{\keywordsAnd}{\and}
\newcommand{\keywords}[1]{\par\noindent{\def\and{\unskip,\ }{\bf Keywords }#1}\par}
\newcommand{\mscclasses}[1]{\par\noindent{\def\and{\unskip,\ }{\bf MSC }#1}\par}

% Algorithm style
\crefname{line}{Step}{Steps} % Do we want to have "Step" or "Line"?
\SetKw{KwOr}{or}
\SetKw{KwAnd}{and}

% https://tex.stackexchange.com/a/42728
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\emailLink}[1]{\textsc{email} \href{mailto:#1}{#1}}
\newcommand{\orcidLink}[1]{\textsc{orcid} \href{https://orcid.org/#1}{#1}}
\newcommand{\amsmscLink}[1]{\href{https://mathscinet.ams.org/mathscinet/msc/msc2020.html?t=#1}{#1}}
\newcommand{\missing}{\textcolor{red}{MISSING}}
\newcommand{\incomplete}{\textcolor{red}{INCOMPLETE}}
\newcommand{\wrong}{\textcolor{red}{WRONG!}}
\newcommand{\TODO}[1]{\textcolor{red}{TODO:~#1}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rinf}{\overline{\R}} 			% \Rinf := \R \cup \{\infty\}
\DeclareMathOperator*{\argmin}{\arg\min}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\proj}{\Pi}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\indicator}{\delta}
\DeclareMathOperator{\support}{\sigma}
\newcommand{\coloneqq}{:=}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator{\stt}{subject~to}
\newcommand{\func}[3]{#1 \colon #2 \to #3}
\newcommand{\ffunc}[3]{#1 \colon #2 \rightrightarrows #3}
\newcommand{\innprod}[2]{\langle #1, #2 \rangle}
\newcommand{\norm}[1]{\Vert #1 \Vert}
\DeclareMathOperator\dist{dist}%											distance
\DeclareMathOperator\epi{epi}%												epigraph
\DeclareMathOperator\closedball{\mathbb{B}}%								closed ball
\DeclareMathOperator\hzn{hzn}%												horizon cone of a function
\newcommand{\conj}{\ast}
\newcommand{\downtoneq}{\downarrow}% \to from above, strictly above
\newcommand{\downto}{\searrow}% \to from above, with possible equality
\newcommand{\nto}{\nrightarrow}% negated \to
\newcommand{\epito}{\xrightarrow[]{\text{e}}}%								epi-convergence
\newcommand{\epimult}{\star}% epi-multiplication
\newcommand{\emphdef}[1]{\textsc{#1}}% emphasis for definitions

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% boxes
\newenvironment{mybox}{}{}

\numberwithin{equation}{section}
\counterwithin{figure}{section}
\counterwithin{table}{section}

\newcommand{\XX}{\R^n}
\newcommand{\YY}{\R^m}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\safeYY}{Y_\textup{sg}}% dual safeguard set
\newcommand{\optiYY}{\mathcal{Y}}% optimal dual set
\newcommand{\multYY}{Y_\textup{mul}}
\newcommand{\dualLL}{\mathpzc{M}}
\newcommand{\hhfun}{\mathpzc{h}}

% https://sronpersonalpages.nl/~pault/#fig:scheme_bright
\definecolor{color_none}{RGB}{221,170,51}%yellow
\definecolor{color_rigid}{RGB}{187,85,102}%red
\definecolor{color_elastic}{RGB}{0,68,136}%blue

\usepackage[normalem]{ulem}
\newcommand{\underdashed}[1]{\dashuline{#1}}
